Duality-based Convex Optimization for Real-time Obstacle Avoidance between Polytopes with Control Barrier Functions

Developing controllers for obstacle avoidance between polytopes is a challenging and necessary problem for navigation in tight spaces. Traditional approaches can only formulate the obstacle avoidance problem as an offline optimization problem. To address these challenges, we propose a duality-based safety-critical optimal control using nonsmooth control barrier functions for obstacle avoidance between polytopes, which can be solved in real-time with a QP-based optimization problem. A dual optimization problem is introduced to represent the minimum distance between polytopes and the Lagrangian function for the dual form is applied to construct a control barrier function. We validate the obstacle avoidance with the proposed dual formulation for L-shaped (sofa-shaped) controlled robot in a corridor environment. We demonstrate real-time tight obstacle avoidance with non-conservative maneuvers on a moving sofa (piano) problem with nonlinear dynamics.

==> sections/case-study1.tex <==
\section{Obstacle Avoidance for Fully Actuated Polytopes}
\label{sec:obstacle-avoidance}

\subsection{Centralized Safety Certificates}

In this section we apply the dual formulation to safe centralized control of $N$ robots, which can translate and rotate in 3D space, and demonstrate how our method allows exact computation of CBF when we have a nominal evading maneuver \cite{squires2018constructive}. The robots have $6$ inputs: $3$ for acceleration of CoM, and $3$ for the angular velocity. We study this problem as an extension to the centralized formulation in \cite{wang2017safety}, where obstacle avoidance is implemented on fully actuated cylindrical robots moving in the 2D plane.

Primarily, in this section we guarantee safety of the overall system by considering a braking maneuver. The CBF is chosen as the square of the minimum distance between two polytopes over the entire braking maneuver, which can provide a guarantee of control invariance for the safe set \cite{squires2018constructive}. We will choose a braking controller such that the square of the minimum distance over the entire trajectory can be computed exactly, thus allowing for tighter tolerances than a method such as in \cite{wang2017safety}.

The state of the $i$-th robot is $\bm{s_i} = (\bm{r_i}, \bm{v_i}, R_i) \in \R^3 \times \R^3 \times SO(3)$, where $\bm{r_i}$ denotes the position vector of the CoM, $\bm{v_i} = \dot{\bm{r}}_{\bm{i}}$, and $R_i$  is the rotation matrix which transforms a vector in some body fixed frame to the ground frame. The inputs are $\bm{u_i} = (\bm{a_i}, \bm{\omega_i}) \in \R^3 \times \R^3$, where $\bm{a_i} = \dot{\bm{v}}_{\bm{i}}$, and $\bm{\omega_i}$ is the angular velocity of the robot represented in the body frame.

The physical boundaries of the $i$-th robot are defined as a polytope around the robot as $\mathcal{P}_i$, which is a function of $\bm{r_i}$ and $R_i$.
\begin{equation} \label{eq:C1-def-poly-0}
\mathcal{P}_i(0,I) \coloneqq \{\bm{x} \in \R^3: A_i\bm{x} \leq b_i, \text{ if } \bm{r_i} = 0, R_i = I\}
\end{equation}

The acceleration and angular velocity of the $i$-th robots is constrained as:
\begin{align} \label{eq:C1-input-lim}
	\lVert \bm{a_i} \rVert_{\infty} \leq \bm{a_i}^{max}\\\nonumber
	\lVert \bm{\omega_i} \rVert_{\infty} \leq \bm{\omega_i}^{max}
\end{align}
The velocity is also constrained as:
\begin{equation} \label{eq:C1-vel-lim}
\lVert \bm{v_i} \rVert_{2} \leq \bm{v_i}^{max}
\end{equation}

\begin{rem}
Since $\mathcal{P}_i(0,I)$ encloses the robot $i$, the CoM of the robot lies inside $\mathcal{P}_i(0,I)$. $\mathcal{P}_i(0,I)$ is defined such the CoM is at the origin $\Rightarrow \; 0 \in \mathcal{P}_i(0,I)$. So, $b_i \geq 0$.
\end{rem}

As the robot translates and rotates, the boundary of the robot changes as follows:
\begin{equation} \label{eq:C1-def-poly-s}
\mathcal{P}_i(\bm{s}) \coloneqq \mathcal{P}_i(\bm{r_i}, R_i) = \{\bm{x} \in \R^3: A_iR_i^T\bm{x} \leq (b_i+A_iR_i^T\bm{r_i})\}
\end{equation}

To construct a CBF, we first consider a safe, braking maneuver $\bm{u_i} = \beta_i(\bm{s_i})$ for all robots as follows:

The maximum time to brake to zero speed from any initial state and for any robot is given by:
\begin{equation} \label{eq:C1-def-TM}
T_M \coloneqq \dfrac{\max_i \bm{v_i}^{max}}{\min_i \bm{a_i}^{max}}
\end{equation}
The braking maneuver is such that the robots to come to rest exactly $T_M$ time after the braking maneuver initiates for all robots. Further, the angular velocity is chosen to be zero. So, the inputs used for the $i$-th robot are ($t=0$ is the time at which the braking maneuver starts):
\begin{equation} \label{eq:C1-brake-maneuver}
\beta_i(\bm{s_i}) = \begin{bmatrix}\bm{a_i} \\ \bm{\omega_i}\end{bmatrix} = \begin{bmatrix}-\frac{\bm{v_i}(0)}{T_M} \\ 0 \end{bmatrix}
\end{equation}

We will derive the controller for two robots $i$ and $j$ for simplicity of notation, however, the controller can easily be generalized to $N$ robots. A CBF is now constructed as \cite{squires2018constructive}:
\begin{equation} \label{eq:C1-def-cbf-inf}
h(\bm{s}) \coloneqq \min_{\tau \in [0,T_M]} \rho(\phi_{\beta}(\tau,\bm{s}(0)))
\end{equation}
where $\bm{s} = (\bm{s_i},\bm{s_j})$, $\phi_{\beta}(\cdot,\cdot)$ is the flow under the braking controller and $\rho(\bm{s})$ is the square of the minimum distance between $\mathcal{S}_i(\bm{s_i})$ and $\mathcal{S}_j(\bm{s_j})$. This formulation guarantees control invariance of the set $\{\bm{s}: h(\bm{s}) \geq 0\}$ \cite{squires2018constructive}. We will show that $h(\bm{s})$ can be computed using a QP.

The velocity of any robot $i$ at time $\tau$ after the braking maneuver starts is:
\begin{equation}
\bm{v_i}(\tau) = \bm{v_i}(0) - \bm{a_i}(\tau)\tau = \bm{v_i}(0)\left(1 - \frac{\tau}{T_M}\right)
\end{equation}
which is proportional to $\bm{v_i}(0)$. The relative velocity of $j$ with respect to $i$ is
\begin{equation} \label{eq:C1-rel-vel}
\bm{v_{ji}}(\tau) = \bm{v_j}(\tau)-\bm{v_i}(\tau) = (\bm{v_j}(0)-\bm{v_i}(0))\left(1 - \frac{\tau}{T_M}\right)
\end{equation}
So, the position of the $j$-th robot relative to the $i$-th robot, $\bm{r_{ji}}$, follows a straight line. The minimum distance during the entire trajectory can now be computed by constructing the convex hull of the trajectory of the $j$-th robot with respect to the $i$-th robot.

So, the minimum distance between robots $i$ and $j$ for $\tau \in [0,T_M]$, is the minimum distance between $\mathcal{S}_i(0,R_i(0))$ and conv$\{\mathcal{S}_j(\bm{r_{ji}}(\tau),R_j(\tau)), \forall \tau \; \in [0,T_M]\} = $ conv$\{\mathcal{S}_j(\bm{r_{ji}}(0),R_j(0)), \mathcal{S}_j(\bm{r_{ji}}(T_M),R_j(0))\}$, where conv $\{ \cdot\}$ represents convex hull of a set. Note that $\tau = 0$ is the time at which the braking maneuver starts and thus represents the current time. The convex hull of polytopes can be represented as a polytope using the relaxation of Balas' Formulation \cite{conforti2014integer}.

\begin{proposition} \label{prop:conv-hull}
The following QP can be used to compute $h(\bm{s})$:
\begin{equation} \label{eq:C1-min-dist-primal}
	\begin{array}{ll@{}ll}
		h(\bm{s}) = & \text{min} \;\;\; & \lVert \bm{x} - \bm{y} \rVert^2_2 &\\[3pt]
		& \text{st} & \bar{A}_i(\bm{s})\bm{x} \leq b_i\\
		& & \bar{A}_j(\bm{s})\bm{y_1} \leq \bar{b}_0(\bm{s})\mu \\
		& & \bar{A}_j(\bm{s})\bm{y_2} \leq \bar{b}_T(\bm{s})(1-\mu) \\
		& & 0 \leq \mu \leq 1 \\
		& & \bm{y} = \bm{y_1} + \bm{y_2} \\
		& & \bm{x}, \bm{y}, \bm{y_1}, \bm{y_2} \in \R^3, \mu \in \R\\
	\end{array}
\end{equation}
The matrices $A_1$, $A_2$, $b_2$, and $b_3$ are computed as:
\begin{align} \label{eq:C1-compact-mat}
	& \bar{A}_i(\bm{s}) = A_iR_i^T \\\nonumber
	& \bar{A}_j(\bm{s}) = A_jR_j^T \\\nonumber
	& \bar{b}_0(\bm{s}) = b_j + A_jR_j^T\bm{r_{ji}} \\\nonumber
	& \bar{b}_T(\bm{s}) = b_j + A_jR_j^T\left[\bm{r_{ji}}+\bm{v_{ji}}\frac{T_M}{2}\right]
\end{align}
\end{proposition}

\begin{proof}
See Appendix \ref{app:proof-conv-hull}
\end{proof}

The Lagrangian function $\Lambda_{ij}(\bm{s},\bm{x},\bm{y_1},\bm{y_2},\bm{y},\mu,\{\bm{\lambda_k}\})$ for \eqref{eq:C1-min-dist-primal} is:
\begin{align} \label{eq:C1-lagrange-func}
\Lambda_{ij} = & \; \lVert \bm{x}-\bm{y} \rVert_2^2 + \bm{\lambda_1}(\bar{A}_i\bm{x}-b_i) + \bm{\lambda_2}(\bar{A}_j\bm{y}_1-\bar{b}_0\mu)\\\nonumber
& + \bm{\lambda_3}(\bar{A}_j\bm{y_2}-\bar{b}_T(1-\mu)) + \bm{\lambda_4}(\mu-1)\\\nonumber
& + \bm{\lambda_5}(-\mu) + \bm{\lambda_6}(\bm{y}-\bm{y_1}-\bm{y_2})
\end{align}
Using the method developed in Section \MakeUppercase{\romannumeral 4}, the Lagrangian dual function for \eqref{eq:C1-min-dist-primal} can explicitly computed by differentiating \eqref{eq:C1-lagrange-func} with respect to $\bm{x}$ and $\bm{y}$ and setting them to zero. Then, the following dual formulation for \eqref{eq:C1-min-dist-primal} can be arrived at:
\begin{equation} \label{eq:C1-min-dist-dual}
	\begin{array}{ll@{}ll}
		-h(\bm{s}) = & \text{min} \;\;\; & \frac{1}{4}\bm{\lambda_6}\bm{\lambda_6}^T + \bm{\lambda_1}b_i + \bm{\lambda_3}\bar{b}_T(\bm{s}) + \bm{\lambda_4} &\\[3pt]
		& \text{st} & \bm{\lambda_1}\bar{A}_i(\bm{s}) + \bm{\lambda_6} = 0\\
		& & \bm{\lambda_2}\bar{A}_j(\bm{s}) - \bm{\lambda_6} = 0\\
		& & \bm{\lambda_3}\bar{A}_j(\bm{s}) - \bm{\lambda_6} = 0\\
		& & -\bm{\lambda_2}\bar{b}_0(\bm{s}) + \bm{\lambda_3}\bar{b}_T(\bm{s}) + \bm{\lambda_4} - \bm{\lambda_5} = 0\\
		& & \bm{\lambda_1}, \bm{\lambda_2}, \bm{\lambda_3}, \bm{\lambda_4}, \bm{\lambda_5} \geq 0 &\\
	\end{array}
\end{equation}

\begin{proposition} \label{prop:optimization}
Eq. \eqref{eq:C1-min-dist-dual} is equivalent to the following QP:
\begin{equation} \label{eq:C1-min-dist-dual-red}
	\begin{array}{ll@{}ll}
		-h(\bm{s}) = & \text{min} \;\;\; & \frac{1}{4}\bm{\lambda_1}A_iA_i^T\bm{\lambda_1}^T + \bm{\lambda_1}b_i + \bm{\lambda_2}\bar{b}_0(\bm{s}) + \bm{\lambda_5} &\\[3pt]
		& \text{st} & \bm{\lambda_1}\bar{A}_i(\bm{s}) + \bm{\lambda_2}\bar{A}_j(\bm{s}) = 0\\[3pt]
		& & \bm{\lambda_2}\bar{A}_j(\bm{s})\bm{v_{ji}}(\bm{s})\frac{T_M}{2} + \bm{\lambda_4} - \bm{\lambda_5} = 0\\[3pt]
		& & \bm{\lambda_1}, \bm{\lambda_2}, \bm{\lambda_4}, \bm{\lambda_5} \geq 0
	\end{array}
\end{equation}
\end{proposition}

\begin{proof}
See Appendix \ref{app:proof-optimization}
\end{proof}

Consider some trajectory $\bm{s}(t)$ and $h(t) \coloneqq h(\bm{s}(t))$ and similarly for others. Let $\{\bm{\lambda_k}^*(t)\}, k \in \mathcal{M} = \{1,2,4,5\}$ be a set of optimal solutions to \eqref{eq:C1-min-dist-dual-red}. Using Prop. \ref{lem:deriv-h-dual-QP}, a lower bound of $\dot{h}(t)$ can be computed as:
\begin{align} \label{eq:C1-deriv-L}
	\dot{L}(t,\{\bm{\lambda_k}^*(t)\},\{\dot{\bm{\lambda}}_{\bm{k}}\}) = & -\frac{1}{2}\bm{\lambda_1}^*(t)A_iA_i^T\dot{\bm{\lambda}}_{\bm{1}}^T - \dot{\bm{\lambda}}_{\bm{1}}b_i\\\nonumber
	& - \dot{\bm{\lambda}}_{\bm{2}}\bar{b}_0(t) - \bm{\lambda_2}^*\dot{\bar{b}}_0(t) - \dot{\bm{\lambda}}_{\bm{5}}
\end{align}
where $\{\dot{\bm{\lambda}}_{\bm{k}}\}$ satisfies the derivatives of the constraints of \eqref{eq:C1-min-dist-dual-red}. Since the derivatives of the matrices are implicit functions of $\bm{u}$, we can define the set of $\bm{u}$ and $\{\dot{\bm{\lambda}}_{\bm{k}}\}$ which satisfy the the derivatives of the constraints of \eqref{eq:C1-min-dist-dual-red} as:
\begin{equation} \label{eq:C1-dual-feasible-set}
	\begin{array}{ll@{}ll}
		\hspace{-5pt} \Phi(t) = \hspace{-5pt} & \{ \bm{u}, \{\dot{\bm{\lambda}}_{\bm{k}}\}: \\[3pt]
		& \;\; \dot{\bm{\lambda}}_{\bm{1}}\bar{A}_i(t) + 	\bm{\lambda_1}^*(t)\dot{\bar{A}}_i(t,\bm{u}) + \dot{\bm{\lambda}}_{\bm{2}}\bar{A}_j(t)\\[3pt]
		& \hspace{20pt} + \bm{\lambda_2}^*(t)\dot{\bar{A}}_j(t,\bm{u}) = 0\\[3pt]
		& \;\; (\dot{\bm{\lambda}}_{\bm{2}}\bar{A}_j(t) + 	\bm{\lambda_2}^*(t)\dot{\bar{A}}_j(t,\bm{u}))\bm{v_{ji}}(t)\frac{T_M}{2} \\[3pt]
		& \hspace{20pt} + \bm{\lambda_2}^*(t)\bar{A}_j(t)\bm{a_{ji}}\frac{T_M}{2} + 	\dot{\bm{\lambda}}_{\bm{4}} - \dot{\bm{\lambda}}_{\bm{5}} = 0\\[3pt]
		& \;\; [\dot{\bm{\lambda}}_{\bm{m}}]_k \geq 0 \;\; \text{if } [\bm{\lambda_m}^*(t)]_k  = 0, \;\forall \; m \in \mathcal{M} \}\\
	\end{array}
\end{equation}
We note that all the constraints are linear in $\bm{u}$ and $\{\dot{\bm{\lambda}}_{\bm{k}}\}$ \eqref{eq:C1-deriv-matrix}.

% \begin{note}
% $\{\bm{\lambda_k}^*(t)\}$ is not required to be continuous. It is only required that at each $t$ a set of right differentiable optimal dual solution exist such as defined in \eqref{eq:family-func-dual}. This allows us to differentiate the constraints of \eqref{eq:5.13}.
% \end{note}

Generalizing to $N$ robots, the following QP is used to compute the input $\bm{u}(t)$ by enforcing CBF constraints on $\dot{L}(t,\{\bm{\lambda_k}^*(t)\},\{\dot{\bm{\lambda}}_{\bm{k}}\},\bm{u})$:
\begin{equation} \label{eq:C1-dual-QP}
	\begin{array}{ll@{}ll}
		\hspace{-5pt} \bm{u}(t) = \hspace{-5pt} & \arg \min_{\{\bm{u},\{\dot{\bm{\lambda}}_{\bm{k}}\}\}} \;\; \lVert \bm{u} - \bm{u}^{nom}(t) \rVert^2_2 &\\[3pt] % + \epsilon(-\sum_{i}\sum_{j>i}\dot{L}_{ij}(t,\{\lambda_k^*(t)\},\{\dot{\lambda}_k\},u)) &\\
		% & \hspace{-6pt} \left. \begin{array}{r@{}l@{}}
		& \text{st \;} \dot{L}(t,\{\bm{\lambda_k}^*(t)\},\{\dot{\bm{\lambda}}_{\bm{k}}\},\bm{u}) \geq -\alpha_2(h(t)-\epsilon^2)\\[3pt]
		& \phantom{st \;\;} ( \bm{u}, \{\dot{\bm{\lambda}}_{\bm{k}}\} ) \in \Phi(t)\\[3pt]
		 % \end{array} \right\rbrace \begin{array}{@{}r@{}l} & \forall \; i,j \\ & j > i \end{array}\\
	    % & \hspace{-6pt} \left. \begin{array}{r@{}l@{}}
		& \phantom{st \;\;} \bm{v_i}^T\bm{a_i} \leq \alpha_3(\lVert \bm{v_i}^{max} \rVert^2_2 - \bm{v_i}^T\bm{v_i})\\[3pt]
		& \phantom{st \;\;} \lVert \bm{a_i} \rVert_{\infty} \leq \bm{a_i}^{max}, \lVert \bm{\omega_i} \rVert_{\infty} \leq \bm{\omega_i}^{max}\\[3pt]
		%  \end{array} \right\rbrace \forall \; i\\
		& \phantom{st \;\;} \bm{v_j}^T\bm{a_j} \leq \alpha_3(\lVert \bm{v_j}^{max} \rVert^2_2 - \bm{v_j}^T\bm{v_j})\\[3pt]
		& \phantom{st \;\;} \lVert \bm{a_j} \rVert_{\infty} \leq \bm{a_j}^{max}, \lVert \bm{\omega_j} \rVert_{\infty} \leq \bm{\omega_j}^{max}
	\end{array}
\end{equation}
where $\bm{u}^{nom}(t)$ is a stabilizing control law as defined in Sec. \ref{sec:background}, $\alpha_2, \alpha_3 > 0$ are constants, and
\begin{align} \label{eq:C1-deriv-matrix}
	\bm{\lambda_1}^*(t)\dot{\bar{A}}_i(t,\bm{u}) = & \bm{\omega_i}^T\widehat{\left(A_i(t)^T\bm{\lambda_1}^*(t)^T\right)}R_i(t)^T\\[3pt]\nonumber
	\bm{\lambda_2}^*(t)\dot{\bar{A}}_j(t,\bm{u}) = & \bm{\omega_j}^T\widehat{\left(A_j(t)^T\bm{\lambda_2}^*(t)^T\right)}R_j(t)^T\\[3pt]\nonumber
	\bm{\lambda_2}^*(t)\dot{\bar{b}}_0(t,\bm{u}) = & \bm{\lambda_2}^*(t)\dot{\bar{A}}_j(t,\bm{u})\bm{r_{ji}}(t) + \bm{\lambda_2}^*(t)\bar{A}_j(t)\bm{v_{ji}}(t)\\[3pt]\nonumber
	\bm{\lambda_2}^*(t)\dot{\bar{b}}_T(t,\bm{u}) = & \bm{\lambda_2}^*(t)\dot{\bar{b}}_0(t,\bm{u}) + \bm{\lambda_2}^*(t)\dot{\bar{A}}_j(t,\bm{u})\bm{v_{ji}}(t)\frac{T_M}{2}\\[3pt]\nonumber
	& + \bm{\lambda_2}^*(t)\bar{A}_j(t)\bm{a_{ji}}\frac{T_M}{2}
\end{align}
Here, the variables $\{\bm{\lambda_k}^*(t)\}$ and $\{\dot{\bm{\lambda}}_{\bm{k}}\}$ are defined separately for each pair $i-j$ of robots, and $\hat{\cdot}: \R^3 \rightarrow \mathfrak{so}(3)$ is such that $\bm{a} \times \bm{b} = \hat{\bm{a}}\bm{b} \; \forall \; \bm{a},\bm{b} \in \R^3$. Also, similar to Sec. \ref{sec:dual-formulation} we substitute $h(t)$ with $(h(t) - \epsilon^2)$, for a small $\epsilon > 0$. $\epsilon$ is chosen considering the time step of computation, velocity and angular velocity bounds, and diameter of the polytopes.

To generalize \eqref{eq:C1-dual-QP} to $N$ robots, we would need dual variables $\{\bm{\lambda_{ij,k}}^*(t)\}$ for $k \in \mathcal{M}, j > i$, i.e. dual variables for each pair of robots. We would also need $\bar{b}_{ij,0}$ and $\bar{b}_{ij,T}$ for each pair of robots. To write the CBF constraints, we enforce the first two constraints of \eqref{eq:C1-dual-QP} for each pair of robots.

\begin{theorem}[Safety] \label{th3.1}
	Enforcing CBF conditions \eqref{eq:C1-dual-QP} for each pair $i-j$ of the robots guarantees safety of the system in the following sense: If $h(0) \geq \epsilon^2$, then $\rho(t) \geq \epsilon^2 \; \forall \; t \geq 0$.
\end{theorem}

\begin{proof}
We can prove the above result using the following statements:
\begin{enumerate}
    \item $h(\bm{s}) \leq \rho(\bm{s}) \; \forall \; \bm{s}$. If for some state $\bm{s}$ $\bm{v_{ij}} = 0$, then $h(\bm{s}) = \rho(\bm{s})$. Both of these statement are true because of the construction of $h(\bm{s})$ \eqref{eq:C1-def-cbf-inf}, and the braking controller \eqref{eq:C1-brake-maneuver}.
    \item If \eqref{eq:C1-dual-QP} is feasible for $t \in [t_1, t_2]$, and $h(t_1) > \epsilon^2$, then $h(t_2) > \epsilon^2$. This is because if \eqref{eq:C1-dual-QP} is feasible, then $\dot{h}(t) \geq -\alpha_2(h(t)-\epsilon^2)$ as shown in Sec. \ref{sec:dual-formulation}, which then guarantees that $h(t_2) > \epsilon^2$ \cite{ames2019control}.
    \item If \eqref{eq:C1-dual-QP} is infeasible at time $t_1$ and $h(t_1) > \epsilon^2$, then using the braking controller will ensure that $\rho(t) > \epsilon^2 \; \forall \; t \in [t_1,t_1+T_M]$ and $v_{i}(t_1+T_M) = 0 \; \forall \; i$. This is by the construction of the braking controller.
    \item If $\bm{v_i}(t) \geq 0 \; \forall \; i$ and $h(t) \geq \epsilon^2$, \eqref{eq:C1-dual-QP} is feasible. In this case, the zero vector would be feasible.
\end{enumerate}

Since $h(0) > \epsilon^2$, $\rho(0) \geq \epsilon^2$. If \eqref{eq:C1-dual-QP} is feasible for time $[0,t]$, then $\rho(t) \geq h(t) \geq \epsilon^2$. If not, then we can apply the braking controller, and the velocities of all robots will become zero at time $t+T_M$. Then, $h(t+T_M) = \rho(t+T_M) \geq \epsilon^2$ and \eqref{eq:C1-dual-QP} is feasible, and we can repeat the process. So, $\rho(t) \geq \epsilon^2 \; \forall \; t \geq 0$. We note that bounds on speed don't affect safety because the braking controller reduces speed for all robots.

% If the system is safe initially, then $h_{ij}(0) \geq 0$ for all $i,j > i$. Since $h_{ij}$ is defined using a safe, braking maneuver, the set $\mathcal{A}_{ij} = \{(\bm{s_i},\bm{s_j}): \; h_{ij}(\bm{s_i},\bm{s_j}) > 0\}^c$ is control-invariant. So, $\exists \; \bm{u_i},\bm{u_j}$ such that $\dot{h}_{ij}(\bm{s_i},\bm{s_j},\bm{u_i},\bm{u_j}) \geq -\alpha_2h_{ij}(\bm{s_i},\bm{s_j})$ for all $\alpha_2 > 0$ and $(\bm{s_i},\bm{s_j}) \in \mathcal{A}_{ij}$. So, \eqref{eq:C1-dual-QP} (without the velocity consrtaints) is always feasible in $\mathcal{A}_{ij}$.

% So, by the CBF property, $h_{ij}(\bm{s_i}(t),\bm{s_j}(t)) \geq 0$ for all time $t \geq 0$, i.e. each pair $i-j$ of the robots is independently safe.

% Since the braking maneuver for robot $i$ does not depend on the states of the other robots, the braking maneuver is safe for the entire system for all time $t \geq 0$.

\end{proof}

% \begin{theorem} \aks{rewrite}
%	The CBF constraints for bounded velocity does not affect the safety of the system.
% \end{theorem}

%\begin{proof}
%	Let $\mathcal{V}_{i} = \{\bm{s_i}: \; \lVert \bm{v_i} \rVert_2 \leq \bm{v_i}^{max}\}$.
	
%	Then, $\mathcal{A}_{ij} \cap \mathcal{V}_{i} \cap \mathcal{V}_j$ is control invariant. This is because the braking maneuver reduces the magnitude of velocity, so both robots $i$ and $j$ stay within $\mathcal{V}_i$ and $\mathcal{V}_j$ for the entire braking trajectory. So, \eqref{eq:C1-dual-QP} is always feasible in $\mathcal{A}_{ij} \cap \mathcal{V}_{i} \cap \mathcal{V}_j$.
	
% 	Then by Theorem \ref{th3.1}, the overall system is also stable.
% \end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Simulation Results}

In this section, we report simulation results for $N$ fully actuated robots using the centralized controller \eqref{eq:C1-dual-QP}. We also report computation time per iteration, analyse the trend in the size of the QP to be solved, and compare our results with a similar centralized controller for 2D fully actuated cylindrical robots implemented in \cite{wang2017safety}.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.99\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/3d-obs-min-d.png}
        \caption{Minimum distance for different pairs}
        \label{fig:obs-avoid-min-d}
    \end{subfigure}
    \begin{subfigure}[t]{0.99\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{figures/3d-obs-cbf-constraint.png}
        \caption{Control barrier function constraints}
        \label{fig:obs-avoid-cbf-constraint}
    \end{subfigure}
    \caption{Illustration of safety performance of the system. The top plot shows minimum distance between all the pairs of robots over time. The bottom plot shows both the lower bound of $\dot{h}(t)$ and $\dot{h}(t)$ satisfying the CBF constraints, with $\bar{\alpha}_2(t) = -\alpha_2(h(t)-\epsilon^2)$}
\end{figure}

Let $m_M$ be the maximum number of faces for all robots. Then, the number of optimization variables in \eqref{eq:C1-dual-QP} is at most $6N + ^NC_2(2m_M) = 6N + N(N-1)m_M$, the number of inequality constraints is at most $^NC_2(2m_M+3) + 7N$, and the number of equality constraints is at most $4^NC_2$. In addition to the \eqref{eq:C1-dual-QP}, we have to compute $^NC_2$ additional QPs to compute $h(t)$. As $N$ increases, the size of the QP increases quadratically as in the case for 2D cylindrical robots. However, unlike the 2D cylindrical robot case, we have to compute $^NC_2$ additional QPs to compute the minimum distance and optimal dual solutions between each pair of robots.

For our simulations, we consider a combination of tetrahedrons (4 faces) and cubes (6 faces) with a average of around 5 faces. Using $m_M = 5$, Table \ref{table:sim-time} tabulates the number of variables and the maximum number of constraints, and the average computation time per iteration and its standard deviation for $N = 3, 5, 10$. The initial and final positions are chosen randomly from a 3D grid. For our example, the computation time required for $N$ robots is approximately the same as that required for $10N$ robots for the centralized implementation in \cite{wang2017safety}. The simulations are performed on a Windows laptop with a $\SI{2.2}{Ghz}$ Intel Core i7 processor running quadprog on MATLAB.

\begin{table}[h]
    \caption{Size of optimization problem and computation time}
    \label{table:sim-time}
    \centering
    \begin{tabular}{| c | c c c |}
    \hline
     & \multicolumn{3}{c |}{Number of Obstacles} \\ \cline{2-4}
     & $N = 3$ & $N = 5$ & $N = 10$ \\ \hline
    Number of variables & 48 & 130 & 510 \\ \hline
    Total number of constraints & 72 & 205 & 835 \\ \hline
    Mean computation time ($\SI{}{ms}$)& 7 & 15 & 394 \\ \hline
    S.D. of computation time ($\SI{}{ms}$)& 1 & 16 & 513 \\ \hline
    \end{tabular}
\end{table}

For illustration, we consider 2 tetrahedral and 1 cuboidal robot with intersecting nominal trajectories. The margin $\epsilon = \SI{5}{cm}$ and the velocity bound is $\SI{4}{m/s}$. The acceleration and angular velocity bounds are $\SI{1}{m/s^2}$ and $\SI{0.2\pi}{rad/s}$. The average computation time per iteration is $6.8 \; ms$. The minimum distance between robots $i$ and $j$, $d_{ij}(t)$, is computed as $\sqrt{h_{ij}(t)}$. Fig. \ref{fig:obs-avoid-min-d} shows that the minimum distance between each pair of robots approaches close to zero but never equal to it, indicating that the robots are tightly packed at around $t = \SI{10}{s}$. This might not be possible for ellipsoidal over-approximation of the polytopes. Fig. \ref{fig:obs-avoid-cbf-constraint} reaffirms the idea that we can achieve safe control by enforcing CBF constraints on a lower bound of $\dot{h}(t)$. An animation of the motion of the robots can be found at \aks{link}.

We can observe from Table \ref{table:sim-time} that there is a large variation in the computation time, which are observed when either two robots approach zero minimum distance or when there is sudden changes in angular velocity. We speculate that it could be due to optimal solution to \eqref{eq:min-dist-primal} jumping from one vertex to another, causing a discontinuity in $\dot{h}(t)$. As the number of vertices increase, these jumps would increase and at the same time the polytope would become smoother. So, in practice, there is a trade-off between tighter safety tolerances (which can be obtained by considering the robot as a polytope) and computation time (which can be enhanced by considering ellipsoidal over-approximations).

We note the following advantages for our method:
\begin{enumerate}
    \item Any feasible solution of \eqref{eq:C1-dual-QP} guarantees safety of the system. A candidate feasible solution is using the braking controller, i.e. $a_{i} = \beta_i(\bm{s_i}), \dot{\bm{\lambda}}_{\bm{1}}=0, \dot{\bm{\lambda}}_{\bm{2}}=0$, and $\dot{\bm{\lambda}}_{\bm{4}}$ and $\dot{\bm{\lambda}}_{\bm{5}}=0$ are chosen according to \eqref{eq:C1-dual-feasible-set}.
    
    \item The optimization problem is quadratic in cost and linear in constraints even for non-linear systems.
    
    \item Safety can be guaranteed even for tight tolerances around the robot. 
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Implementation Details} \aks{change heading and reduce length}

Several implementation issues were encountered during the simulations. These issues have been listed below:

\begin{enumerate}
    \item \aks{recheck} As noted in Sec. \ref{sec:dual-formulation}, $\dot{h}(t)$ need not be continuous. In our case, since we directly control the angular velocity and there are no rate constraints on it, we can have discontinuity in $\dot{h}(t)$ when the optimal solution of \eqref{eq:min-dist-primal} jumps from one vertex to another. This can be seen in \aks{graph} at \aks{around} $t = $. The polytopes can intersect due to large bounds on angular velocity, large polytopes, or large time steps in the simulation.
    
    \item \aks{recheck} The (possibly) discontinuous nature of the control law can lead to discrete-time sliding behaviour such as \aks{around} $t = $ in \aks{figure}, where the state rapidly oscillates around the region of discontinuity. Also, the non-Lipschitz form of the feedback control law can significantly increase simulation time.
    
    \item For large number of objects, the numerical solution may return infeasible solutions, resulting in unsafe motion and subsequent collision.
    
    \item Since $h(t) \geq 0 \; \forall \; t$, the control is not robust in the sense that if the system leaves the unsafe set, it may not converge back to the safe set. Control barrier functions have the property that if the system leaves the safe set, it will converge back to it.
\end{enumerate}


==> sections/case-study2.tex <==
\section{Example: Non-convex Obstacle Avoidance}
\label{sec:non-convex-obs-avoid}

% \begin{figure}%[!htp]
%    \centering
%    \includegraphics[width=1.0\linewidth]{figures/3d-obs-avoid-traj.png}
%    \caption{Trajectories of centre of mass for three obstacles over a duration of $\SI{100}{s}$. The CBF formulation for polytopes was used for safety and CLF for reference tracking. \aks{add animation link}}
%    \label{fig:obs-avoid-traj}
% \end{figure}

In this section, we show that the duality based formulation \eqref{eq:dual-QP} can be used for safe control of non-convex obstacles in tightly constrained environments. The specific problem we consider is of navigating a non-convex L-shaped robot through a L-shaped corridor. The control inputs to the robot are its 2D velocity and angular velocity.

The state of the robot is $\bm{s} = (\bm{p},\theta) \in \R^2 \times \R$. The control inputs are $\bm{u} = (\bm{v},\omega)$, such that $\dot{\bm{p}} = \bm{v}$ and $\dot{\theta} = \omega$. The inputs are bounded as $\lVert \bm{v} \rVert_\infty \leq \bm{v}^{max}$ and $|\omega| \leq \omega^{max}$.

The corridor is represented in the form of rectangles $\mathcal{O}_j, j\in \{1,2,3\}$, and the robot is represented as two rectangles $\mathcal{S}_i, i\in \{1,2\}$. The width of the corridor is $1 \; m$ and the side length of the robot is $1.1 \; m$. So, we have to use the non-convex structure of the robot to navigate through the corridor.

The CBF is chosen as the square of minimum distance, and the CBF constraints are enforced between the polytopes $\mathcal{O}_i$ and $\mathcal{P}_j$ for $i \in \{1,2,3\}, j \in \{1,2\}$. We note that the robot will remain safe since the allowable set is control invariant (we can choose $\bm{v} = 0, \omega = 0$). The stabilizing controller $\bm{u}^{nom}(t)$ is enforced as a CLF constraint with a slack term, and the desired point as the end of the corridor.

Snapshots the robot moving through the corridor are shown in Fig. \ref{fig:snapshots-sofa-problem}. MPT3 \cite{MPT3} and the IPOPT package \cite{wachter2006implementation} for MATLAB were used for illustration and optimization respectively.
